Learning and scoring Gaussian latent variable causal models with unknown additive interventions

With observational data alone, causal structure learning is a challenging problem. The task becomes easier when having access to data collected from perturbations of the underlying system, even when the nature of these is unknown. Existing methods either do not allow for the presence of latent variables or assume that these remain unperturbed. However, these assumptions are hard to justify if the nature of the perturbations is unknown. We provide results that enable scoring causal structures in the setting with additive, but unknown interventions. Specifically, we propose a maximum-likelihood estimator in a structural equation model that exploits system-wide invariances to output an equivalence class of causal structures from perturbation data. Furthermore, under certain structural assumptions on the population model, we provide a simple graphical characterization of all the DAGs in the interventional equivalence class. We illustrate the utility of our framework on synthetic data as well as real data involving California reservoirs and protein expressions. The software implementation is available as the Python package \emph{utlvce}.

==> algorithm.tex <==
\section{Practical use cases of \methName{}}
\label{sec:optimization}
We next describe how \methName{} can be used in practice to account for latent effects and obtain a set of DAGs that fit the data well. In Section~\ref{sec:alternating}, we propose an alternating minimization strategy to solve \eqref{eqn:est2_marg} with the DAG, hence also the support of $B$, {being} pre-specified. Building on this, in Section~\ref{sec:alg_candidate_dags}, we consider the setting where a candidate set of DAGs are available (for example as for the protein expressions dataset in Section~\ref{sec:experiments}) and describe how \methName{} can be used to obtain an optimally scoring equivalence class of DAGs. Finally, in Section~\ref{sec:alg_starting_point}, we extend our algorithmic framework to the setting when a set of DAGs represent starting points, and we deploy \methName{} to improve on these DAGs by removing any spurious dependencies. A python package containing the implementation of all components of \methName{} is available at \url{https://github.com/juangamella/ut-lvce}.
% A
%TensorFlow implementation of CoRe as well as code to reproduce some of the experimental results are available at https://github.com/christinaheinze/core.
%Finally, in Section~\ref{sec:validation}, we 

We remark here that searching for optimally scoring DAGs (according to the score \eqref{eqn:score}) is a very difficult computational task. In particular, an immediate approach that comes to mind is to develop a greedy DAG search over the space of equivalent models akin to GES \cite{chick02}. Indeed, \cite{GamellaGnies2021} develops a greedy algorithm to move in the space of interventionally equivalent DAGs for the model \eqref{eq:SCM_env} \emph{without} latent variables. By employing the \methName{} score function \eqref{eqn:score}, one may adapt the method of \cite{GamellaGnies2021} to incorporate latent effects. However, a significant conceptual challenge is that the likelihood score \eqref{eqn:score} is not decomposable according to the DAG structure due to latent confounding; the lack of score decomposability renders greedy-based techniques computationally expensive. Thus, our focus in this paper is to demonstrate the utility of \methName{} on the use cases described in the previous paragraph.

%{\bf{Setup for running synthetic example}:} For our numerical illustrations in this section, we consider a collection of $p = 20$ observed variables influenced by $h=2$ latent variables. The entries of the latent coefficient matrix $\Gamma^\star \in \mathbb{R}^{p \times h}$ are generated IID from the distribution $\mathcal{N}(0,1/\sqrt{p})$. The noise term $\epsilon_i$ for each coordinate $i$ is distributed according to $\epsilon_i \sim \mathcal{N}(0,\zeta_i)$ where $\xi_i$ is chosen uniformly and independently from the interval $[0.5,0.6]$. We suppose there are $m = 5$ environments, where $\delta^{e}$ is all zeros for $e = 1$ and for the environments $e = 2,3,\dots,5$ and every $i \in I^\star$, $\delta^{e}_i \sim \mathcal{N}(0,\zeta_i)$ where $\zeta_i$ is chosen uniformly and independently from the interval $[6,10]$. Here, $I^\star \subset [p]$ consists of $10$ indices chosen at random. Finally, for every environment $e = 1,2,\dots,5$ and $i \in [h]$, the latent variables are distributed according to $H^e_i \sim \mathcal{N}(0,\zeta_i)$ where $\zeta_i$ is chosen uniformly and independently from the interval $[0.5,0.6]$. The population connectivity matrix $B^\star$ and the amount of data in every environment are specified later. 
 
%Finally, in \suppmat{} Section~\ref{sec:additional_synthetic}, we provide additional experiments for the following settings: weaker interventions on observed variables, stronger latent effects and larger number of latent variables. 

%In particular, a significant conceptual challenge is that the likelihood score \eqref{eqn:score} is not decomposable according to the DAG structure due to latent confounding; the lack of score decomposability renders greedy-based techniques computationally expensive. 

%searching over the space of DAGs in the presence of latent variables is a very challenging task. In particular, a prospective  

%A naive idea is to search over the space of DAGs, which is known to be very challenging and in some sense NP-hard \citep{hardndess}. A more reasonable approach is to develop a greedy DAG search over the space of equivalent models akin to GES \cite{chick02}. Indeed, \cite{GamellaGnies2021} develops a greedy algorithm to move in the space of interventionally equivalent DAGs for the model \eqref{eq:SCM_env} \emph{without} latent variables. By employing the \methName{} score function   \eqref{eqn:score}, one may adapt the method of \cite{GamellaGnies2021} to incorporate latent effects. However, a significant conceptual challenge is that the likelihood score \eqref{eqn:score} is not decomposable according to the DAG structure due to latent confounding; the lack of score decomposability renders greedy-based techniques computationally expensive. 

%are not available, and present some computational heuristics for structure search over different DAGs.

%Solving the \methName{} estimator \eqref{eqn:est2_marg} for a fixed DAG is a key ingredient for evaluating different DAGs in a candidate set. Thus, we first propose an optimization procedure to solve \eqref{eqn:est2_marg} with the DAG, hence also the support of $B$, pre-specified. 
%In Section~\ref{sec:alg_structural_learning}, we extend our algorithmic framework to the setting when candidate DAGs are not available. We propose a 
%we extend the previous framework to allow


%Solving the \methName{} estimator \eqref{eqn:est2_marg} for a DAG $\dagg$ is a challenging task, as the problem is non-convex over the decision variables $(B,\Gamma,\{\Omega_{e},\Psi_e\}_{e = 1}^m)$. Further, searching over the space of DAGs is super-exponential in the number of variables. These computational challenges are common in causal structure learning problems and are made {worse}
%worst 
%with the presence of multiple environments and latent confounding. In this section, we propose some heuristics for computing \methName{} {based on perturbation data} to find optimal scoring DAGs;
%given perturbation data; 
%we discuss open questions regarding computations involving the \methName{} in Section~\ref{section:discussion}. The outline of this section is as follows: in Section~\ref{section:dag_score}, we describe a method to compute \methName{} for a given DAG structure, that is, when the support of $B$ is pre-specified. Building on this, in Section~\ref{section:potential_dags}, we describe some computational heuristics for structure search over different DAGs. 


%\begin{equation}
%\begin{aligned}
 %  & \lambda_{B}:= \lambda~~;~~~\lambda_{I} := \lambda\gamma \\
  %  &\texttt{score}_{\lambda_{B},\lambda_{I}}(\dagg,\hat{\Theta}(\dagg,\bar{h})) := \sum_{e = 1}^{m}\hat{\pi}_e\ell(\hat{B},\hat{\Gamma},\hat{\Omega}_e,\hat{\Psi}_e;\hat{\Sigma}_{e}) + \lambda_{B}(\|\dagg\|_{\ell_0}+p\texttt{degree}(\text{moral}(\dagg))) + \lambda_{I}|\hat{I}|.
%\end{aligned}
%\end{equation}
\subsection{Alternating minimization strategy to compute the \methName{} estimator}
\label{sec:alternating}
We first describe an optimization approach for solving \methName{} given an input DAG $\dagg$ and a fixed intervention target set $I$. Our optimization algorithm is based on the following alternating minimization strategy: starting with an initialization of all of the model parameters, we fix $B$ and perform gradient updates to find updated estimates for the parameters $(\Gamma,\{\Omega_e,\Psi_e\}_{e=1}^m$ where the noise variances $\{\Omega_e\}_{e=1}^m$ are compatible with the input intervention set $I$, and then update $B$ by solving a convex program to optimality with the remaining parameters fixed. We find that the alternating method described above is relatively robust to the initialization scheme, but we nonetheless propose the following concrete strategy:
\begin{equation}
\begin{aligned}
1)~&B^{(0)}  \text{ via linear regression with pooled data}, \\
2)~&\Gamma^{(0)} = UD^{1/2} \text{ where } UDU^T \text{ is SVD of } (\id-B^{(0)})\hat{\Sigma}_\text{pooled}(\id-B^{(0)})^T, \\
3)~& \Omega_e^{(0)} = \texttt{diag}\left\{(\id-B^{(0)})\hat{\Sigma}_\text{pooled}(\id-B^{(0)})^T\right\} \text{ for }e\in[m], \\
4)~& \Psi_e^{(0)} = \mathrm{Id} \text{ for } e \in [m],
\end{aligned}
\label{eqn:init}
\end{equation}
 where $\hat{\Sigma}_{\text{pooled}}$ is the covariance matrix of the pooled data. The first step follows since the DAG structure is known. The entire procedure, involving the initialization step and the parameter updates, is presented in Algorithm \ref{algo:dag_score}.
 \setcounter{algorithm}{-1}
\begin{algorithm}[]
\caption{Solving \methName{} to score a given DAG $\dagg$ for a fixed $(
\lambda,\gamma,\bar{h})$}
\begin{algorithmic}[1]
\vspace{0.1in}
\STATE {\bf Input}: DAG $\dagg$; intervention targets ${I}$; data $\hat{\Sigma}_e$, $\hat{\pi}_e$ for $e \in [m]$; regularization params. $\lambda,\gamma \geq 0$; $\#$ of latent vars. $\bar{h}$
\vspace{.05in}
\STATE{\bf Initialize parameters}: via relation \eqref{eqn:init}
\vspace{0.04in}
\STATE{\bf Alternating minimization}: solve for causal parameters
\begin{itemize}
	\item[(a)] fixing $(\Gamma^{(t)}, \{(\Omega_e^{(t)},\Psi_e^{(t)})\}_{e = 1}^m)$, update $B^{(t+1)}$ by solving {the} convex optimization program \eqref{eqn:est2_marg} where $B^{(t+1)}$ is compatible with $\dagg$. Fixing $B^{(t+1)}$, perform gradient updates until convergence to find $(\Gamma^{(t+1)}, \{(\Omega_{e}^{(t+1)},\Psi_e^{(t+1)})\}_{e = 1}^m)$ where $\Omega_{e}^{(t+1)}$ is compatible with ${I}$
    \item[(b)] perform alternating iterates for positive integers $t$ until convergence at iteration $T$
    \item[(c)] obtain estimates $\hat{\Theta}(\dagg,\bar{h}):= (\hat{B}^{(T)},\hat{\Gamma}^{(T)},{I},\{(\hat{\Omega}_e^{(T)},\hat{\Psi}_e^{(T)})\}_{e=1}^m)$ %and add $\hat{\Theta}(\dagg,\bar{h})$ to $\hat{\Theta}_{\text{cand}}$
    %\item[(d)] Remove the variable with weakest estimated intervention: $\hat{I} \leftarrow \hat{I} \setminus \{\min_{i \in \hat{I}} \log(\frac{1}{m}\sum_{e=1}^m[\hat{\Omega}_e]_{i,i})-\frac{1}{m}\sum_{e=1}^m\log([\hat{\Omega}_e]_{i,i})\}$
     \end{itemize}
\vspace{0.04in}
\STATE{\bf Output:} causal parameters $\hat{\Theta}(\dagg,\bar{h})$ and regularized likelihood $\texttt{score}_{\lambda,\gamma}(\dagg,\hat{\Theta}(\dagg,\bar{h}))$
%the likelihood score $\min_{\hat{\Theta}(\dagg,\bar{h})\in \Theta_\text{cand}} \texttt{score}(\dagg,\hat{\Theta}(\dagg,\bar{h}))$ and the associated minimizer
\end{algorithmic} \label{algo:dag_score}
\end{algorithm}
%The gradients for step 3(a) of Algorithm \ref{algo:dag_score} are provided in \suppmat{} Section~\ref{sec:supp_mat_gradients}. 
Step 3(b) involves two convergence criteria: the convergence of the gradient steps for the parameters $(\Gamma^{(t)},\{(\Omega_{e}^{(t)},\Psi_e^{(t)})\}_{e = 1}^m)$ as well as the convergence of the alternating procedure. For the first criterion, we terminate the gradient descent when the relative change in the likelihood score is below $\epsilon_1$. For the second criterion, we terminate the alternating minimization at step $T$ when $\|B^{(T)}-B^{(T-1)}\|_\infty \leq \epsilon_2$. In our numerical experiments, we set $\epsilon_1 = 10^{-6}$ and $\epsilon_2 = 10^{-2}$. 




\begin{comment}
\begin{algorithm}
\caption{Equivalence class of best scoring DAGs from a candidate set via \methName{}} 
\begin{algorithmic}[1]
\vspace{0.1in}
\STATE {\bf Input}: candidate DAG(s) $\dagg_\text{cand}$; data $\hat{\Sigma}_e,\hat{\pi}_e$ for $e \in[m]$; regularization params. $\lambda,\gamma \geq 0$; $\#$ of latent vars. $\bar{h}$
\vspace{.05in}
\STATE{\bf Obtain likelihood score for each DAG}: for each $\dagg \in \dagg_\text{cand}$, supply $(\dagg,{I} = [p])$ to Algorithm~\ref{algo:dag_score} to obtain the causal parameters $\hat{\Theta}(\dagg,\bar{h})$ and $\texttt{score}_{\lambda,\gamma}(\dagg,\hat{\Theta}(\dagg,\bar{h}))$
\vspace{0.05in}
\STATE{\bf Find an optimally scoring DAG}: obtain ${\dagg}_\text{opt} = \arg\min_{\dagg \in \dagg_\text{cand}} \texttt{score}_{\lambda,\gamma}(\dagg,\hat{\Theta}(\dagg,\bar{h}))$%. Let $\{\hat{\Omega}_e\}_{e=1}^m$ be noise variance encoded in  $\hat{\Theta}(\dagg_\text{opt},\bar{h})$
\vspace{0.05in}
%\STATE{\bf Estimate intervention strengths}: compute $\xi_j := \log(\frac{1}{m}\sum_{e=1}^m[\hat{\Omega}_e]_{j,j})-\frac{1}{m}\sum_{e=1}^m\log([\hat{\Omega}_e]_{j,j})$ for each $j \in [p]$
%\vspace{0.05in}
\STATE{\bf Greedy backward deletion to estimate intervention targets}: initialize $\hat{I} = I$ and%etting $\{\hat{\Omega}_e\}_{e=1}^m$ be noise variance encoded in $\hat{\Theta}(\dagg_\text{opt},\bar{h})$
\begin{enumerate}
%\item[(a)] initialize $\hat{I}_\dagg = [p]$
\item[(a)] let $\{\hat{\Omega}_e\}_{e=1}^m$ be noise variance encoded in $\hat{\Theta}(\dagg_\text{opt},\bar{h})$
\item[(b)] estimate intervention strengths via $\xi_j := \frac{1}{m}\sum_{e=1}^m([\hat{\Omega}_e]_{j,j}-\frac{1}{m}\sum_{e=1}^m [\hat{\Omega}_e]_{j,j})^2$ for each $j \in [p]$
\item[(c)] remove the variable with weakest estimated intervention: $\hat{I} \leftarrow \hat{I} \setminus \{\arg\min_{j \in \hat{I}}\xi_j\}$
\item[(d)] supply $(\dagg_\text{opt},\hat{I})$ as input to Algorithm~\ref{algo:dag_score} to obtain likelihood $\texttt{score}_{\lambda,\gamma}(\dagg,\hat{\Theta}(\dagg_\text{opt},\bar{h}))$
\item[(e)] repeat (c,d) until likelihood score does not improve
\end{enumerate}
%\vspace{0.05in}
%\STATE{\bf Estimate connectivity matrices:} for every $\dagg \in \hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg_\text{opt})$%, supply ${\dagg}$ and $\hat{I}$ to Algorithm~\ref{algo:dag_score} to obtain connectivity matrix $\hat{B}_{{\dagg}}$ encoded in the estimate $\hat{\Theta}({\dagg},\bar{h})$%for every $\dagg \in \dagg_\text{opt}$ and every $\bar{\dagg}\in \hat{I}_\dagg\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg)$, supply $\bar{\dagg}$ and $\hat{I}_\dagg$ to Algorithm~\ref{algo:dag_score} to obtain connectivity matrix $\hat{B}_{\bar{\dagg}}$ encoded in the estimate $\hat{\Theta}(\bar{\dagg},\bar{h})$
\vspace{0.05in}
\STATE{\bf Output:} equivalence class $\hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg_\text{opt})$ using Definition~\ref{defn:equiv_class} %and connectivity matrices $\hat{B}_\dagg$ for every $\dagg \in \hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg_\text{opt})$
%equivalence class of DAGs and corresponding connectivity matrices $\{(\bar{\dagg},B_{\bar{\dagg}}) \text{ where }\bar{\dagg} \in \hat{I}_\dagg\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg) \text{ for some }\dagg \in \dagg_\text{opt}\}$% 
%$\{\hat{I}_\dagg\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg) \text{ for every }\dagg\in\dagg_\text{opt}$ and connectivity matrices $\hat{B}_{\dagg}$ for every $\dagg \in \hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg_\text{opt})$
\end{algorithmic} \label{algo:equiv_class}
\end{algorithm}
\end{comment}



%%The parameters $(\lambda,\gamma,\bar{h})$ index 
%\noindent{\emph Remark 6:} Note that 
%Since the scoring procedure in Algorithm~\ref{algo:2} involves some heuristics and there may be multiple DAGs that yield an optimal score, one may more conservatively choose ``near" optimal scoring DAGs in step 4 of Algorithm~\ref{algo:dag_score}. Second, since the candidate DAGs $\dagg_\text{cand}$ may be overly dense due to the latent effects, the optimal connectivity matrix $\hat{B}_\text{opt}$ may consist of weak but nonzero spurious edges. In our numerical experiments in Section~\ref{section:experiments}, we find the optimally scoring DAG(s) (using \methName{}) among $\dagg_\text{cand}$. Then, for each optimal DAG, we remove each of its edges (in the reverse order of their edge strength) and compute the likelihood score of the resulting DAG (using \methName{}). We then choose the DAG(s) that obtain the smallest likelihood score along the entire path. 

%While the optimization program \eqref{eqn:est2_marg} is jointly non-convex, solving for the connectivity matrix $B$ with the nuisance parameters $\Gamma,\{\Psi_e\}_{e=1}^m,$ and $\{\Omega_{e}\}_{e=1}^m$ fixed is a convex program. Since we are mainly interested in an accurate estimate for the connectivity matrix, we propose the following alternating minimization strategy: starting with an initialization of all of the model parameters, we fix $B$ and perform gradient updates to find updated estimates for the nuisance parameters, and then update $B$ -- by solving a convex program to optimality with the remaining parameters fixed.


%Finally, we discuss the selection of hyperparameters $(\lambda,\gamma,\bar{h})$ in the subsequent section. 
\subsection{Using \methName{} to identify the best scoring DAGs from a candidate set}
\label{sec:alg_candidate_dags}
Let $\dagg_\text{cand}$ be a candidate set of DAGs (potentially a singleton). Building on Algorithm~\ref{algo:dag_score}, we present an algorithm to identify an optimally scoring DAG as well as DAGs in its equivalence class. First, using Algorithm~\ref{algo:dag_score}, we score each DAG in the candidate set with $I = [p]$, and obtain an optimally scoring DAG $\dagg_\text{opt}$ with noise variances $\{\hat{\Omega}_e\}_{e=1}^m$. To estimate the intervention targets $\hat{I}$, we measure the variation in each coordinate of $\hat{\Omega}_e$ across the environments as large variations indicate that the corresponding variable has received an intervention. To quantify the degree of variation, we compute a ``variance like" metric $\xi_j := \frac{1}{m}\sum_{e=1}^m([\hat{\Omega}_e]_{j,j}-\frac{1}{m}\sum_{e=1}^m [\hat{\Omega}_e]_{j,j})^2$ for each $j \in \hat{I}$ (also defined in Section~\ref{sec:known_latent_perturb}), where large values of $\xi_j$ provide stronger evidence for the presence of an intervention on variable $X_j$. We propose a systematic approach to estimate an intervention set $\hat{I}$ using the values $\xi_j$: we greedily remove the variable with the smallest variation $\xi_j$ and compute the regularized likelihood with the resulting intervention set. We repeat this process until the likelihood score can no longer be improved. Thus, as output, we return the equivalence class of optimally scoring DAGs $\hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg_\text{opt})$. A detailed summary of our procedure is presented in Algorithm~\ref{algo:equiv_class}.
%Finally, for every $\dagg \in \hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg_\text{opt})$, we supply $(\dagg,\hat{I})$ to Algorithm~\ref{algo:dag_score} to compute a corresponding connectivity matrix $\hat{B}_\dagg$.  and the corresponding connectivity matrices

\begin{algorithm}
\caption{Equivalence class of best scoring DAGs from a candidate set via \methName{}} 
\begin{algorithmic}[1]
\vspace{0.1in}
\STATE {\bf Input}: candidate DAG(s) $\dagg_\text{cand}$; data $\hat{\Sigma}_e,\hat{\pi}_e$ for $e \in[m]$; regularization params. $\lambda,\gamma \geq 0$; $\#$ of latent vars. $\bar{h}$
\vspace{.05in}
\STATE{\bf Obtain likelihood score for each DAG}: for each $\dagg \in \dagg_\text{cand}$, supply $(\dagg,{I} = [p])$ to Algorithm~\ref{algo:dag_score} to obtain the causal parameters $\hat{\Theta}(\dagg,\bar{h})$ and $\texttt{score}_{\lambda,\gamma}(\dagg,\hat{\Theta}(\dagg,\bar{h}))$
\vspace{0.05in}
\STATE{\bf Find an optimally scoring DAG}: obtain ${\dagg}_\text{opt} = \arg\min_{\dagg \in \dagg_\text{cand}} \texttt{score}_{\lambda,\gamma}(\dagg,\hat{\Theta}(\dagg,\bar{h}))$%. Let $\{\hat{\Omega}_e\}_{e=1}^m$ be noise variance encoded in  $\hat{\Theta}(\dagg_\text{opt},\bar{h})$
\vspace{0.05in}
%\STATE{\bf Estimate intervention strengths}: compute $\xi_j := \log(\frac{1}{m}\sum_{e=1}^m[\hat{\Omega}_e]_{j,j})-\frac{1}{m}\sum_{e=1}^m\log([\hat{\Omega}_e]_{j,j})$ for each $j \in [p]$
%\vspace{0.05in}
\STATE{\bf Greedy backward deletion to estimate intervention targets}: initialize $\hat{I} = I$ and%etting $\{\hat{\Omega}_e\}_{e=1}^m$ be noise variance encoded in $\hat{\Theta}(\dagg_\text{opt},\bar{h})$
\begin{enumerate}
%\item[(a)] initialize $\hat{I}_\dagg = [p]$
\item[(a)] let $\{\hat{\Omega}_e\}_{e=1}^m$ be noise variance encoded in $\hat{\Theta}(\dagg_\text{opt},\bar{h})$
\item[(b)] estimate intervention strengths via $\xi_j := \frac{1}{m}\sum_{e=1}^m([\hat{\Omega}_e]_{j,j}-\frac{1}{m}\sum_{e=1}^m [\hat{\Omega}_e]_{j,j})^2$ for each $j \in [p]$
\item[(c)] remove the variable with weakest estimated intervention: $\hat{I} \leftarrow \hat{I} \setminus \{\arg\min_{j \in \hat{I}}\xi_j\}$
\item[(d)] supply $(\dagg_\text{opt},\hat{I})$ as input to Algorithm~\ref{algo:dag_score} to obtain likelihood $\texttt{score}_{\lambda,\gamma}(\dagg,\hat{\Theta}(\dagg_\text{opt},\bar{h}))$
\item[(e)] repeat (c,d) until likelihood score does not improve
\end{enumerate}
%\vspace{0.05in}
%\STATE{\bf Estimate connectivity matrices:} for every $\dagg \in \hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg_\text{opt})$%, supply ${\dagg}$ and $\hat{I}$ to Algorithm~\ref{algo:dag_score} to obtain connectivity matrix $\hat{B}_{{\dagg}}$ encoded in the estimate $\hat{\Theta}({\dagg},\bar{h})$%for every $\dagg \in \dagg_\text{opt}$ and every $\bar{\dagg}\in \hat{I}_\dagg\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg)$, supply $\bar{\dagg}$ and $\hat{I}_\dagg$ to Algorithm~\ref{algo:dag_score} to obtain connectivity matrix $\hat{B}_{\bar{\dagg}}$ encoded in the estimate $\hat{\Theta}(\bar{\dagg},\bar{h})$
\vspace{0.05in}
\STATE{\bf Output:} equivalence class $\hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg_\text{opt})$ using Definition~\ref{defn:equiv_class} %and connectivity matrices $\hat{B}_\dagg$ for every $\dagg \in \hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg_\text{opt})$
%equivalence class of DAGs and corresponding connectivity matrices $\{(\bar{\dagg},B_{\bar{\dagg}}) \text{ where }\bar{\dagg} \in \hat{I}_\dagg\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg) \text{ for some }\dagg \in \dagg_\text{opt}\}$% 
%$\{\hat{I}_\dagg\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg) \text{ for every }\dagg\in\dagg_\text{opt}$ and connectivity matrices $\hat{B}_{\dagg}$ for every $\dagg \in \hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg_\text{opt})$
\end{algorithmic} \label{algo:equiv_class}
\end{algorithm}
\noindent{\emph Remark 4:} The guarantees of Theorems~\ref{thm:sparse_dense} and Theorem~\ref{thm:perturbed_latent_known} can be extended to Algorithm~\ref{algo:equiv_class}. Specifically, suppose the conditions of either of these theorems hold and the candidate set of DAGs $\dagg_{\text{cand}}$ contains a member of the population interventional equivalence class, i.e. $\dagg_{\text{cand}} \cap {I}^\star\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}({\dagg}^\star) \neq \emptyset$. Furthermore, suppose that Algorithm~\ref{algo:dag_score} obtains a globally optimal solution; indeed, this is guaranteed if the initial parameters in \eqref{eqn:init} are sufficiently close to the population parameters. Then, in the infinite data limit, the output of Algorithm~\ref{algo:equiv_class} is consistent, i.e. $\hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg_\text{opt}) = {I}^\star\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}({\dagg}^\star)$ with high probability as the number of samples in each environment tends to infinity.

\noindent\textbf{Selecting $(\lambda,\gamma,\bar{h})$ via cross-validation:} In \suppmat{} Section~\ref{sec:supp_mat_cross_validation}, we propose an approach to exhaustively search over the equivalence classes indexed by $(\lambda,\gamma,\bar{h})$, and choose an optimal one based on validation with test data. The complexity of our validation approach is $\approx \tilde{t}((\bar{h}_\text{max}+1)|{\dagg}_{\text{cand}}| + p)$, where $\bar{h}_\text{max}$ is the maximum number of latent variables allowed in the model and $\tilde{t}$ represents the time it takes to score a DAG using Algorithm~\ref{algo:dag_score}. The value for $\tilde{t}$ depends on the DAG and the data generating mechanism; in our numerical experiments, this is typically on the order of $5$ seconds for $p = 20$ node graphs.

%As an illustration for the computational speed of this validation scheme, 

%for the computational speed of performing cross-validation to select all tuning parameters, after supplying $10$ randomly generated DAGs of $p = 20$ nodes with average degree \Armeen{Put this number} as input to Algorithm~\ref{algo:equiv_class}, the cross-validated output is computed in approximately \Armeen{PUT THIS NUMBER}. 
%All of our numerical experiments are performed with this cross-validation procedure.
%We thoroughly analyze the computational speed (as well as statistical performance) of our procedure in Section~\ref{sec:experiments}.
%We illustrate the utility of Algorithm~\ref{algo:structure_learning} using the synthetic setup described earlier. Let the population DAG $\dagg^\star$ be an Erd{\"o}s-renyi graph with average degree $2$ and edge strengths $0.7$.  The candidate set of DAGs are taken to be the Markov equivalence class of $\dagg^\star$, which by definition is a superset of the interventional equivalence class $I^\star\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}({\dagg}^\star)$. We generate $n$ observations for each environment, where $n$ is chosen from the set $\{500,1000,10000\}$. To illustrate the effectiveness of the scoring function, we supply the data and each candidate DAG, with $I = [p]$ to Algorithm~\ref{algo:dag_score}. The left plot in Figure~\ref{fig:equivalence_class_recovery}a displays the proportion of instances, across $50$ independent trials, that the best scoring DAG is inside $I^\star\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}({\dagg}^\star)$. We observe that as the sample size increases, the scoring function becomes more accurate and correctly outputs a member of the interventional equivalence class. In order to obtain an equivalence class of best scoring DAGs, we apply Algorithm~\ref{algo:equiv_class}. As shown in the right plot in Figure~\ref{fig:equivalence_class_recovery}a, the estimated equivalence class is close to the true equivalence class.  

%\begin{figure}
%    \centering
%        \subfigure[Best scoring DAGs using Algorithm~\ref{algo:equiv_class}]{
 %       \includegraphics[scale = 0.47]{images/plot_1.pdf}}
 %        \subfigure[Removing spurious edges using  Algorithm~\ref{algo:structure_learning}]{
 %       \includegraphics[scale = 0.55]{images/plot_baseline_3_final.pdf}}
 %   \caption{Illustration with the synthetic setting: a) proportion of instances, among $50$ independent trials, that the best scoring DAG in Step 3 of Algorithm~\ref{algo:equiv_class} is in $I^\star\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}({\dagg}^\star)$ and average $\mathrm{FDP}$ and $\mathrm{TDP}$ of the estimated $\hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg^\star)$; b) performance of Algorithm~\ref{algo:structure_learning} with the `starting point' DAGs $\mathrm{MEC}(\dagg^\star) + \text{20 random edges}$.} 
%        \label{fig:equivalence_class_recovery}
%\end{figure}
%%The parameters $(\lambda,\gamma,\bar{h})$ index 
%\noindent{\emph Remark 6:} Note that 
%Since the scoring procedure in Algorithm~\ref{algo:2} involves some heuristics and there may be multiple DAGs that yield an optimal score, one may more conservatively choose ``near" optimal scoring DAGs in step 4 of Algorithm~\ref{algo:dag_score}. Second, since the candidate DAGs $\dagg_\text{cand}$ may be overly dense due to the latent effects, the optimal connectivity matrix $\hat{B}_\text{opt}$ may consist of weak but nonzero spurious edges. In our numerical experiments in Section~\ref{section:experiments}, we find the optimally scoring DAG(s) (using \methName{}) among $\dagg_\text{cand}$. Then, for each optimal DAG, we remove each of its edges (in the reverse order of their edge strength) and compute the likelihood score of the resulting DAG (using \methName{}). We then choose the DAG(s) that obtain the smallest likelihood score along the entire path. 

%While the optimization program \eqref{eqn:est2_marg} is jointly non-convex, solving for the connectivity matrix $B$ with the nuisance parameters $\Gamma,\{\Psi_e\}_{e=1}^m,$ and $\{\Omega_{e}\}_{e=1}^m$ fixed is a convex program. Since we are mainly interested in an accurate estimate for the connectivity matrix, we propose the following alternating minimization strategy: starting with an initialization of all of the model parameters, we fix $B$ and perform gradient updates to find updated estimates for the nuisance parameters, and then update $B$ -- by solving a convex program to optimality with the remaining parameters fixed.
\subsection{Using \methName{} to remove spurious edges from `starting point' DAGs}
\label{sec:alg_starting_point}
We next consider settings where the DAGs in a candidate set are viewed as `starting points' and may contain spurious dependencies due to potential latent confounding. Such scenarios naturally arises in practice. For example, a domain expert may be unsure about some of the edges in a DAG and may include them in the analysis to be conservative. In other contexts, the user may have deployed their favorite structure learning algorithm(s) to obtain a set of DAGs. Since many of the computationally efficient structural learning approaches (e.g. GES) do not account for the presence of latent variables, the fitted graph may be more dense than the population DAGs. 

Our objective, in contexts where DAGs are viewed as starting points, is to use \methName{} to remove spurious dependencies and return a refined set of equally scoring DAGs. Our approach is based on the following simple observation: scoring starting point DAGs using Algorithm~\ref{algo:dag_score} may yield connectivity matrices that are more dense than the population connectivity matrix, although the magnitude of the spurious edges will be small. To remove these spurious edges, for each DAG in the candidate set, we greedily delete the weakest edge and compute a regularized likelihood score using Algorithm~\ref{algo:dag_score}. We repeat this process until the score can no longer be improved. After pruning, we obtain a refined collection of candidate DAGs, which are then supplied to Algorithm~\ref{algo:equiv_class} to identify an optimally scoring set of DAGs. A summary of the entire procedure is presented in Algorithm~\ref{algo:structure_learning}. Similar to Algorithm~\ref{algo:equiv_class}, in all our numerical experiments, we choose the regularization parameters $(\lambda,\gamma,\bar{h})$ via cross-validation; see \suppmat{} Section~\ref{sec:supp_mat_cross_validation}. The complexity of our exhaustive validation approach is $\approx \tilde{t}((\bar{h}_\text{max}+1)[\sum_{\dagg \in \tilde{\dagg}_{\text{cand}}} \|\dagg\|_{\ell_0}]+ p)$.


%We next consider the setting where a candidate set of DAGs is not available a-priori. To obtain a set of optimally scoring DAGs, there are few approaches one can take. A naive idea is to search over the space of DAGs, which is known to be very challenging and in some sense NP-hard \citep{hardndess}. A more reasonable approach is to develop a greedy DAG search over the space of equivalent models akin to GES \cite{chick02}. Indeed, \cite{GamellaGnies2021} develops a greedy algorithm to move in the space of interventionally equivalent DAGs for the model \eqref{eq:SCM_env} \emph{without} latent variables. By employing the \methName{} score function   \eqref{eqn:score}, one may adapt the method of \cite{GamellaGnies2021} to incorporate latent effects. However, a significant conceptual challenge is that the likelihood score \eqref{eqn:score} is not decomposable according to the DAG structure due to latent confounding; the lack of score decomposability renders greedy-based techniques computationally expensive. 

%To circumvent the aforementioned challenges, we propose a computationally efficient approach to obtain a collection of candidate DAGs; these are then scored via Algorithm~\ref{algo:equiv_class} to identify an equivalence class of optimally scoring DAGs. In particular, we first run GES on the pooled data (without accounting for latent variables) with the following heuristic reasoning:
%\begin{equation}
 %   \text{there exists }\dagg \in \widehat{\text{MEC}} \text{ such that } \dagg^\star \subseteq \dagg
  %  \label{eqn:intuition_dense}
%\end{equation}
%Here, $\widehat{\text{MEC}}$ is the Markov equivalence class obtained by the GES algorithm and the notation $\dagg^\star \subseteq \dagg$ indicates $\dagg^\star$ is a sub-graph of $\dagg$. The intuition behind \eqref{eqn:intuition_dense}  is that fitting a DAG without taking into account the effect of latent variables yields a denser graph compared to the population or Markov equivalent DAGs) since marginalization of latent variables induces confounding dependencies. 

%Thus, scoring such DAGs using Algorithm~\ref{algo:dag_score} may yield connectivity matrices that are more dense than the population connectivity matrix, although the magnitude of the spurious edges will be small. To remove these spurious edges, for each DAG in the estimated Markov equivalence class, we greedily delete the weakest edge and compute a regularized likelihood score using Algorithm~\ref{algo:dag_score}. We repeat this process until the score can no longer be improved. After pruning, we obtain a collection of candidate DAGs, which are then supplied to Algorithm~\ref{algo:equiv_class} to identify an optimally scoring set of DAGs. A summary of the entire procedure is presented in Algorithm~\ref{algo:structure_learning}.


%{Searching over all DAGs is typically not possible unless the number of observed variables $p$ is small. In fact,} performing a combinatorial search is known to be very challenging and in some sense NP-hard \citep{hardness}. {One could rely on greedy strategies \citep{chick02}; we discuss below a strategy which exploits a reasonable set of candidate DAGs.} In the previous section, a set of plausible DAGs was considered. Without this knowledge however, this candidate set must be obtained from data. %Performing a combinatorial search is known to be very challenging and in some sense NP-hard \cite{hardness}. 
%In this section, we propose a heuristic to identify a collection of candidate DAGs to be scored via Algorithm~\ref{algo:equiv_class}. Our approach is to identify these DAGs by assuming no latent confounding. In general, fitting a DAG without taking into account the effect of latent variables yields a denser graph (compared to the population or Markov equivalent DAGs) since marginalization of latent variables induces confounding dependencies. As such, scoring such DAGs using Algorithm~\ref{algo:2} may yield connectivity matrices that are more dense than the population connectivity matrix, although the magnitude of the spurious edges will be small. In our numerical experiments in Section~\ref{section:experiments}, we find the optimally scoring DAG(s) (using \methName{}) among the candidate DAGs. Then, for each optimal DAG, we perform backward deletion by removing each of its edges (in the reverse order of their edge strength) and computing the likelihood score of the resulting DAGs (using \methName{}). We then choose the DAG(s) that obtain the smallest likelihood score along the entire path. 
%We note that one can also perform greedy deletion approaches where edges of the optimal DAGs in the optimal set are removed in a greedy fashion until the score can no longer be improved. %Thus, simply looking at the strongest edges or a crude thresholding of the entries of the connectivity matrices may compensate for the overly dense candidate DAGs {, or one could also do some backward deletion from scored DAGs resulting to consider sub-DAGs of the candidate set.} 

%In Section~\ref{section:intro}, we outlined procedures to identify DAGs without latent confounding, with the constraint based PC algorithm, score based GES, and the hybrid method ARGES being among the most popular for structure learning in the observational setting. In principal, when domain expertise is not available, many of these methods can be used to find candidate DAGs. For simplicity, in our synthetic illustrations in Section~\ref{section:experiments}, we perform GES on pooled environmental data. The GES procedure greedily adds or deletes edges in the space of Markov equivalent DAGs based on $\ell_0$ regularized likelihood score and is asymptotically consistent \citep{chick02}. We select the regularization parameter to be twice the {analogue from the} BIC score (as was suggested in \cite{Nowzohour}). Algorithm~\ref{algo:dag_score} presents the entire procedure of finding candidate DAGs, scoring them, and selecting the final output. 


%We remark that the $\arg\max$ in steps 3 and 5 of Algorithm~\ref{algo:3} may not be unique in the infinite sample limit, due to potential non-identifiability. In practice, the optimization is done to find all optimal DAGs within a relative tolerance value from the minimum (set at $10^{-3}$ in our experiments), and outputs also its several associated parameter estimates.
\begin{algorithm}
\caption{{{}Improving `starting point' DAGs via \methName{}}}
\begin{algorithmic}[1]
\vspace{0.1in}
\STATE {\bf Input}: data $\hat{\Sigma}_e,\hat{\pi}_e$ for $e \in [m]$; candidate DAG(s) $\tilde{\dagg}_\text{cand}$; regularization params. $\lambda,\gamma \geq 0$; $\#$ of latent vars. $\bar{h}$
\vspace{.05in}
%\STATE{\bf Score each DAG}: For each $\dagg \in \dagg_\text{cand}$, supply data and $\hat{I} = [p]$ to Algorithm~\ref{algo:dag_score} to obtain the causal parameter $\hat{\Theta}(\dagg,\bar{h})$
%\vspace{0.05in}
%\STATE{\bf Optimally scoring candidate DAG(s)}: obtain $\tilde{\dagg}_\text{opt} = \arg\max_{\dagg \in \dagg_\text{cand}}\texttt{score}_{\lambda,\gamma}(\dagg,\hat{\Theta}(\dagg,\bar{h}))$
%\vspace{0.05in}
\STATE{\bf Backward deletion to remove spurious edges}: initialize $\dagg_\text{cand} = \emptyset$; for each ${\dagg} \in \tilde{\dagg}_\text{cand}$:
\begin{enumerate}
    \item[(a)] supply data and $(\dagg,\hat{I} = [p])$ to Algorithm~\ref{algo:dag_score} to obtain the score $\texttt{score}_{\lambda,\gamma}({\dagg},\hat{\Theta}(\dagg,\bar{h}))$
    \item[(b)] let ${\dagg}$ be the DAG after deleting the smallest edge in magnitude in ${\dagg}$
    \item[(c)] repeat (a-b) until likelihood score does not improve;  add $\dagg$ to $\dagg_\text{cand}$
\end{enumerate}
\vspace{0.05in}
\STATE{\bf Output}: supply $\dagg_\text{cand}$ to Algorithm~\ref{algo:equiv_class} to obtain an equivalence class of best scoring DAGs %$\hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg_\text{opt})$%best scoring DAGs %and associated connectivity matrices
\end{algorithmic} \label{algo:structure_learning}
\end{algorithm}
\noindent{\emph Remark 5:} As with Remark 4, the guarantees of Theorems~\ref{thm:sparse_dense} and Theorem~\ref{thm:perturbed_latent_known} can be extended to Algorithm~\ref{algo:structure_learning}. In particular, if the candidate set of DAGs $\dagg_{\text{cand}}$ contains a DAG that is a supergraph of a DAG in the population interventional equivalence class, then, in the infinite data limit, the output of Algorithm~\ref{algo:structure_learning} is consistent, i.e. with high probability,  $\hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg_\text{opt}) = {I}^\star\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}({\dagg}^\star)$ as the sample size tends to infinity. 
%For illustration,  we consider the synthetic setting described earlier but generate two different population DAGs $\dagg^\star$: a chain graph with edge strengths $0.7$ and an Erd{\"o}s-renyi graph with average degree $2.1$ and edge strengths $0.7$. In each case, the `starting point' DAGs are taken to be ones in $\mathrm{MEC}(\dagg^\star)$ with $20$ edges at random to each graph (picked uniformly, without replacement, from all valid edge additions). We supply the data and the starting point DAGs to Algorithm~\ref{algo:structure_learning}. Ideally, Algorithm~\ref{algo:structure_learning} removes spurious edges and improves upon the original set of DAGs to identify a class of best scoring DAGs that is close to the population interventional equivalence class. Figure~\ref{fig:equivalence_class_recovery}b confirms this to be the case. In particular, we observe that the estimated interventional equivalence class, averaged across $10$ independent trials, has small average $\mathrm{FDP}$ and large average $\mathrm{TDP}$. Furthermore, we see that as compared to the ``starting point DAGs", Algorithm~\ref{algo:structure_learning} produces an estimate with substantially smaller $\mathrm{FDP}$ without much loss in $\mathrm{TDP}$.


%A few remarks regarding Algorithm~\ref{algo:dag_score} are in order. Since the scoring procedure in Algorithm~\ref{algo:2} involves some heuristics and there may be multiple DAGs that yield an optimal score, one may more conservatively choose ``near" optimal scoring DAGs in step 4 of Algorithm~\ref{algo:dag_score}. Second, since the candidate DAGs $\dagg_\text{cand}$ may be overly dense due to the latent effects, the optimal connectivity matrix $\hat{B}_\text{opt}$ may consist of weak but nonzero spurious edges. In our numerical experiments in Section~\ref{section:experiments}, we find the optimally scoring DAG(s) (using \methName{}) among $\dagg_\text{cand}$. Then, for each optimal DAG, we remove each of its edges (in the reverse order of their edge strength) and compute the likelihood score of the resulting DAG (using \methName{}). We then choose the DAG(s) that obtain the smallest likelihood score along the entire path. 

%%We note that one can also perform greedy deletion approaches where edges of the optimal DAGs in the optimal set are removed in a greedy fashion until the score can no longer be improved. 



%A few remarks regarding Algorithm~\ref{algo:dag_score} are in order. Since the scoring procedure in Algorithm~\ref{algo:2} involves some heuristics and there may be multiple DAGs that yield an optimal score, one may more conservatively choose ``near" optimal scoring DAGs in step 4 of Algorithm~\ref{algo:dag_score}. Second, since the candidate DAGs $\dagg_\text{cand}$ may be overly dense due to the latent effects, the optimal connectivity matrix $\hat{B}_\text{opt}$ may consist of weak but nonzero spurious edges. In our numerical experiments in Section~\ref{section:experiments}, we find the optimally scoring DAG(s) (using \methName{}) among $\dagg_\text{cand}$. Then, for each optimal DAG, we remove each of its edges (in the reverse order of their edge strength) and compute the likelihood score of the resulting DAG (using \methName{}). We then choose the DAG(s) that obtain the smallest likelihood score along the entire path. 

%%We note that one can also perform greedy deletion approaches where edges of the optimal DAGs in the optimal set are removed in a greedy fashion until the score can no longer be improved. 










\begin{comment}
\subsection{Using \methName{} to recover the equivalence class of a given DAG}
Let $\dagg$ be a given DAG. Building on Algorithm~\ref{algo:dag_score}, we present a procedure to identify an equivalence class of DAGs that fit the data equally well. First, using Algorithm~\ref{algo:dag_score}, we score $\dagg$ with $I = [p]$, and obtain latent variable causal model with noise variances $\{\hat{\Omega}_e\}_{e=1}^m$. To estimate the intervention targets $\hat{I}$, we measure the variation in each coordinate of $\hat{\Omega}_e$ across the environments as large variations indicate that the corresponding variable has received an intervention. To quantify the degree of variation, we compute a `variance like' metric $\xi_j := \frac{1}{m}\sum_{e=1}^m([\hat{\Omega}_e]_{j,j}-\frac{1}{m}\sum_{e=1}^m [\hat{\Omega}_e]_{j,j})^2$ for every $j \in [p]$, where large values of $\xi_j$ provide stronger evidence for the presence of an intervention on variable $X_j$. We propose a systematic approach to estimate an intervention set $\hat{I}$ using the values $\xi_j$: we greedily remove the variable with the smallest variation $\xi_j$ and compute the regularized likelihood with the resulting intervention set. We repeat this process until the likelihood score can no longer be improved. Thus, as output, we return the equivalence class of optimally scoring DAGs $\hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg)$. A detailed summary of our procedure is presented in Algorithm~\ref{algo:equiv_class}.

\begin{algorithm}
\caption{Equivalence class of a given DAG via \methName{}} 
\begin{algorithmic}[1]
\vspace{0.1in}
\STATE {\bf Input}: DAG $\dagg$; data $\hat{\Sigma}_e,\hat{\pi}_e$ for $e \in[m]$; regularization params. $\lambda,\gamma \geq 0$; $\#$ of latent vars. $\bar{h}$
\vspace{.05in}
\STATE{\bf Obtain a causal model}: supply $(\dagg,{I} = [p])$ to Algorithm~\ref{algo:dag_score} to obtain the causal parameters $\hat{\Theta}(\dagg,\bar{h})$% and $\texttt{score}_{\lambda,\gamma}(\dagg,\hat{\Theta}(\dagg,\bar{h}))$
\vspace{0.05in}
\STATE{\bf Greedy backward deletion to estimate intervention targets}: initialize $\hat{I} = I$ and%etting $\{\hat{\Omega}_e\}_{e=1}^m$ be noise variance encoded in $\hat{\Theta}(\dagg_\text{opt},\bar{h})$
\begin{enumerate}
%\item[(a)] initialize $\hat{I}_\dagg = [p]$
\item[(a)] let $\{\hat{\Omega}_e\}_{e=1}^m$ be noise variance encoded in $\hat{\Theta}(\dagg,\bar{h})$
\item[(b)] estimate intervention strengths via $\xi_j := \frac{1}{m}\sum_{e=1}^m([\hat{\Omega}_e]_{j,j}-\frac{1}{m}\sum_{e=1}^m [\hat{\Omega}_e]_{j,j})^2$ for each $j \in [p]$
\item[(c)] remove the variable with weakest estimated intervention: $\hat{I} \leftarrow \hat{I} \setminus \{\arg\min_{j \in \hat{I}}\xi_j\}$
\item[(d)] supply $(\dagg,\hat{I})$ as input to Algorithm~\ref{algo:dag_score} to obtain likelihood $\texttt{score}_{\lambda,\gamma}(\dagg,\hat{\Theta}(\dagg,\bar{h}))$
\item[(e)] repeat (c,d) until likelihood score does not improve
\end{enumerate}
%\vspace{0.05in}
%\STATE{\bf Estimate connectivity matrices:} for every $\dagg \in \hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg_\text{opt})$%, supply ${\dagg}$ and $\hat{I}$ to Algorithm~\ref{algo:dag_score} to obtain connectivity matrix $\hat{B}_{{\dagg}}$ encoded in the estimate $\hat{\Theta}({\dagg},\bar{h})$%for every $\dagg \in \dagg_\text{opt}$ and every $\bar{\dagg}\in \hat{I}_\dagg\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg)$, supply $\bar{\dagg}$ and $\hat{I}_\dagg$ to Algorithm~\ref{algo:dag_score} to obtain connectivity matrix $\hat{B}_{\bar{\dagg}}$ encoded in the estimate $\hat{\Theta}(\bar{\dagg},\bar{h})$
\vspace{0.05in}
\STATE{\bf Output:} equivalence class $\hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg)$ using Definition~\ref{defn:equiv_class} %and connectivity matrices $\hat{B}_\dagg$ for every $\dagg \in \hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg_\text{opt})$
%equivalence class of DAGs and corresponding connectivity matrices $\{(\bar{\dagg},B_{\bar{\dagg}}) \text{ where }\bar{\dagg} \in \hat{I}_\dagg\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg) \text{ for some }\dagg \in \dagg_\text{opt}\}$% 
%$\{\hat{I}_\dagg\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg) \text{ for every }\dagg\in\dagg_\text{opt}$ and connectivity matrices $\hat{B}_{\dagg}$ for every $\dagg \in \hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg_\text{opt})$
\end{algorithmic} \label{algo:equiv_class}
\end{algorithm}





%First, using Algorithm~\ref{algo:dag_score}, we score each DAG in the candidate set with $I = [p]$, and obtain an optimally scoring DAG $\dagg_\text{opt}$ with noise variances $\{\hat{\Omega}_e\}_{e=1}^m$. To estimate the intervention targets $\hat{I}$, we measure the variation in each coordinate of $\hat{\Omega}_e$ across the environments as large variations indicate that the corresponding variable has received an intervention. To quantify the degree of variation, we compute a ``variance like" metric $\xi_j := \frac{1}{m}\sum_{e=1}^m([\hat{\Omega}_e]_{j,j}-\frac{1}{m}\sum_{e=1}^m [\hat{\Omega}_e]_{j,j})^2$ for every $j \in [p]$, where large values of $\xi_j$ provide stronger evidence for the presence of an intervention on variable $X_j$. We propose a systematic approach to estimate an intervention set $\hat{I}$ using the values $\xi_j$: we greedily remove the variable with the smallest variation $\xi_j$ and compute the regularized likelihood with the resulting intervention set. We repeat this process until the likelihood score can no longer be improved. Thus, as output, we return the equivalence class of optimally scoring DAGs $\hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg_\text{opt})$. A detailed summary of our procedure is presented in Algorithm~\ref{algo:equiv_class}.
\noindent\textbf{Selecting $(\lambda,\gamma,\bar{h})$ via holdout-validation:} In \suppmat{} Section~\ref{sec:supp_mat_cross_validation}, we propose an efficient approach to search over the equivalence classes indexed by $(\lambda,\gamma,\bar{h})$, and choose an optimal one based on validation with test data. We thoroughly analyze the computational speed (as well as statistical performance) of our procedure in Section~\ref{sec:experiments}. As an illustration, after supplying $10$ randomly generated DAGs of $p = 20$ nodes with average degree \Armeen{Put this number} as input to Algorithm~\ref{algo:equiv_class}, the cross-validated output is computed in approximately \Armeen{PUT THIS NUMBER}. 

\noindent{\emph Remark 4:} The guarantees of Theorems~\ref{thm:sparse_dense} and Theorem~\ref{thm:perturbed_latent_known} can be extended to Algorithm~\ref{algo:equiv_class}. Specifically, suppose the conditions of either of these theorems hold and $\dagg^\star \in {I}^\star\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}({\dagg}^\star)$. Furthermore, suppose that Algorithm~\ref{algo:dag_score} obtains a globally optimal solution; indeed, this is guaranteed if the initial parameters in \eqref{eqn:init} are sufficiently close to the population parameters). Then, in the infinite data limit, the output of Algorithm~\ref{algo:equiv_class} is consistent, i.e. $\hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg_\text{opt}) = {I}^\star\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}({\dagg}^\star)$ with high probability.




To illustrate the utility of Algorithm~\ref{algo:equiv_class}, we consider the setup described at the beginning of Section~\ref{sec:optimization} and let $\dagg^\star$ be an Erd{\"o}s-renyi graph with average degree $2$ and edge strengths $0.7$. We generate $n$ observations for each environment, where $n$ is chosen from the set $\{100,500,1000,10000\}$. We supply the data and $\dagg^\star$ to Algorithm~\ref{algo:equiv_class} to estimate the population interventional equivalence class $I^\star\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg)$. Figure~\ref{fig:equivalence_class_recovery} shows the average $\mathrm{FDP}$ and $\mathrm{TDP}$ (see \eqref{eqn:metrics}) associated with the estimated interventional equivalence class across $50$ independent runs. Since smaller values of $\mathrm{FDP}$ and larger values of $\mathrm{TDP}$ are indicative of better performance, we observe that our procedure produces accurate estimates of the interventional Markov equivalence class.


\begin{figure}
    \centering
    \subfigure{
        \includegraphics[scale = 0.45]{images/plot_1_part2.pdf}}
        \subfigure{
        \includegraphics[scale = 0.45]{images/plot_1_par1.pdf}}
        \subfigure{
        \includegraphics[scale = 0.45]{images/plot_1_part2.pdf}}
        \subfigure{
        \includegraphics[scale = 0.53]{images/plot_baseline_3_fina.pdf}}
    \caption{Performance of Algorithm~\ref{algo:dag_score}: a) proportion of instances, among $50$ independent trials, that the best scoring DAG is in $I^\star\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}({\dagg}^\star)$; b) type-I and type-II errors of the estimated $\hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\hat{\dagg})$.} 
        \label{fig:equivalence_class_recovery}
\end{figure}


\subsection{Using \methName{} to recover an equivalence class of optimally scoring causal models from a set of input DAGs}
\label{sec:alg_candidate_dags}
We next consider the setting where a user has access to multiple DAGs: these may be available from domain knowledge or obtained by any structural learning algorithm. Naturally, the following questions arise: i) what is the best scoring DAG and does  




candidate set of DAGs $\dagg_\text{cand}$ are available. These may be viewed 



Let $\dagg_\text{cand}$ be a candidate set of DAGs (potentially a singleton). Building on Algorithm~\ref{algo:dag_score}, we present an algorithm to identify an optimally scoring DAG as well as DAGs in its equivalence class. First, using Algorithm~\ref{algo:dag_score}, we score each DAG in the candidate set with $I = [p]$, and obtain an optimally scoring DAG $\dagg_\text{opt}$ with noise variances $\{\hat{\Omega}_e\}_{e=1}^m$. To estimate the intervention targets $\hat{I}$, we measure the variation in each coordinate of $\hat{\Omega}_e$ across the environments as large variations indicate that the corresponding variable has received an intervention. To quantify the degree of variation, we compute a ``variance like" metric $\xi_j := \frac{1}{m}\sum_{e=1}^m([\hat{\Omega}_e]_{j,j}-\frac{1}{m}\sum_{e=1}^m [\hat{\Omega}_e]_{j,j})^2$ for every $j \in [p]$, where large values of $\xi_j$ provide stronger evidence for the presence of an intervention on variable $X_j$. We propose a systematic approach to estimate an intervention set $\hat{I}$ using the values $\xi_j$: we greedily remove the variable with the smallest variation $\xi_j$ and compute the regularized likelihood with the resulting intervention set. We repeat this process until the likelihood score can no longer be improved. Thus, as output, we return the equivalence class of optimally scoring DAGs $\hat{I}\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}(\dagg_\text{opt})$. A detailed summary of our procedure is presented in Algorithm~\ref{algo:equiv_class}.



To illustrate the effectiveness of the scoring function, we supply the data and each candidate DAG, with $I = [p]$ to Algorithm~\ref{algo:dag_score}. Figure~\ref{fig:equivalence_class_recovery}a displays the proportion of instances, across $50$ independent trials, that the best scoring DAG is inside $I^\star\hspace{-0.02in}-\hspace{-0.02in}\mathrm{MEC}({\dagg}^\star)$. We observe that as the sample size increases, the scoring function becomes more accurate and correctly outputs a member of the interventional equivalence class. In order to obtain an equivalence class of best scoring DAGs, we apply Algorithm~\ref{algo:equiv_class}. As shown in Figure~\ref{fig:equivalence_class_recovery}b, the estimated equivalence class is close to the true equivalence class.  





\end{comment}
